Hierarchical Indexing for Retrieval-Augmented Opinion Summarization

We propose a method for unsupervised abstractive opinion summarization, that combines the attributability and scalability of extractive approaches with the coherence and fluency of Large Language Models (LLMs). Our method, HIRO, learns an index structure that maps sentences to a path through a semantically organized discrete hierarchy. At inference time, we populate the index and use it to identify and retrieve clusters of sentences containing popular opinions from input reviews. Then, we use a pretrained LLM to generate a readable summary that is grounded in these extracted evidential clusters. The modularity of our approach allows us to evaluate its efficacy at each stage. We show that HIRO learns an encoding space that is more semantically structured than prior work, and generates summaries that are more representative of the opinions in the input reviews. Human evaluation confirms that HIRO generates significantly more coherent, detailed and accurate summaries.

==> ch7-hiro.tex <==
\chapter{The LLM Era: Opinion Summarisation with Hierarchical Indexing}
\label{ch:hiro}

\todo{Compile evidence that we don't need large models? Compare to 1B/50B and show there's no diff?}

\todo{Maybe generate using Hercules clusters + LLM and show that it's worse?}
\todo{Try asking for citations with a prompt}

\todo{Could add HIRO + Llama as an ablation. or discuss qualitatively why we didnt use it}

% \todo{Add lead in from prev chapter (and LLM background)}

In \Cref{ch:hercules} we showed how HRQ-VAE can be used to perform opinion summarization, with the discrete hierarchical representation enabling us to generate summaries that are attributable and scale to large numbers of input reviews. However, the discrete bottleneck used for \textsc{Hercules} must perform two functions: it must group together topically related sentences so that we can identify popular opinions; and, it must also contain sufficiently detailed information about the input sentence that the decoder is able to generate a meaningful reconstruction. These objectives are in opposition with each other, and so \textsc{Hercules} is prone to generating overly generic output and often hallucinates. 

Throughout the thesis so far, we have found that LLMs are able to generate highly fluent output, albeit at the cost of large parameter counts, expensive training and inference, and limited context window lengths. In this chapter, we seek to combine the best properties of generalised LLMs and specialised models that use structured representations, by performing \textit{content selection} in a discrete hierarchical space and using a LLM for the `last mile' generation subtask.

We propose a method for unsupervised abstractive opinion summarization, that combines the attributability and scalability of extractive approaches with the coherence and fluency of Large Language Models (LLMs). Our method, HIRO, learns an index structure that maps sentences to a path through a semantically organized discrete hierarchy. At inference time, we populate the index and use it to identify and retrieve clusters of sentences containing popular opinions from input reviews. Then, we use a pretrained LLM to generate a readable summary that is grounded in these extracted evidential clusters. The modularity of our approach allows us to evaluate its efficacy at each stage. We show that HIRO learns an encoding space that is more semantically structured than prior work, and generates summaries that are more representative of the opinions in the input reviews. Human evaluation confirms that HIRO generates more coherent, detailed and accurate summaries that are significantly preferred by annotators compared to prior work.




\section{Introduction}
\label{sec:intro}



Online review websites are a useful resource when choosing which hotel to visit or which product to buy, but it is impractical for a user to read hundreds of reviews. Automatic opinion summarization aims to aggregate a large and diverse set of customer reviews about a particular \textit{entity} into a single, easy to read summary. A good summary should accurately reflect the balance of opinions in the input reviews, highlighting the most common or \textit{popular} opinions, while omitting unnecessary details. A useful summary should also help \textit{compare} between competing options, and include points that differentiate the current entity from others.

% Early work on opinion summarization extracted reviewers' sentiment about specific features \citep{10.1145/1014052.1014073} or identified salient sentences based on centrality \citep{lexrank}, while more recent methods have proposed \emph{extractive} models that use learned feature spaces  \citep{angelidis-etal-2021-extractive,basu-roy-chowdhury-etal-2022-unsupervised}. 

Some prior work on \emph{abstractive} opinion summarization has almost exclusively either required costly supervision \citep{brazinskas-etal-2021-learning,cattan-etal-2023-key} or has assumed that the number of input reviews is limited \citep{coavoux-etal-2019-unsupervised,brazinskas-etal-2020-unsupervised,amplayo-etal-2021-aspect, amplayo2021unsupervised,iso-etal-2021-convex-aggregation}. This defeats the point of a summary: a user could feasibly read 8 reviews in a reasonable period of time. A good summarization system should be \textit{scalable}, since popular products online may receive thousands of reviews. It should also be \textit{attributable}, offering some evidence to justify its output. Finally, it should generate summaries that are \textit{coherent} and \textit{faithful} to the input reviews.

Large Language Models (LLMs) have been shown to generate highly fluent summaries in the news domain \citep{bhaskar-etal-2023-prompted} but are a flawed solution because current instruction-tuned models are not attributable, and because their context windows limit the number of reviews they are able to base their summaries on. Models with long context windows have been proposed \citep{Beltagy2020Longformer,s4} but these are not currently instruction-tuned, and it has been shown that LLMs are biased toward information at the start and end of the input \citep{liu2023lost}.
% Moreover,  are not attributable.
% and retrieval is beneficial anyway \citep{xu2023retrieval}.

Our approach, \textbf{H}ierarchical \textbf{I}ndexing for \textbf{R}etrieval-Augmented \textbf{O}pinion Summarization (HIRO), identifies informative sentences using hierarchical indexing and then passes the selected sentences as input to a LLM, similar to retrieval-augmented generation \cite[RAG,][]{rag}. This separation of concerns (selection and generation) allows us to combine the attributability and scalability of the discrete representation with the strong generative abilities of LLMs, leading both to a higher quality index and to more informative and coherent output summaries. 

HIRO consists of three modules, allowing for increased control, flexibility and interpretability. The \textbf{Hierarchical Indexer} is an encoder that maps sentences from reviews to paths through a hierarchical discrete latent space. The \textbf{Retriever} uses the index to identify clusters of sentences for each entity that contain popular and informative opinions. These sentence clusters are passed to a \textbf{Generator}, a pretrained LLM, that generates coherent summaries that are grounded in the retrieved sentences.

Our contributions are as follows:
\begin{itemize}
  % \setlength\itemsep{-0.2em}
  % \vspace{-0.2cm}
  \item We propose a method for learning an encoder that maps sentences to a path through a semantically structured discrete hierarchy.
  \item We show how to exploit this discrete hierarchy at inference time to identify clusters of related and prevalent sentences from input reviews.
  \item We introduce an automatic metric that measures whether generated summaries reflect the input reviews, while penalizing overly generic statements.
  \item Through extensive experiments on two English datasets from different product domains, we demonstrate that passing these retrieved sentences in a zero-shot manner to a pretrained LLM generates summaries that better reflect the distribution of opinions within the input reviews. Human evaluation shows that summaries generated by HIRO are significantly more coherent and accurate than prior work, and are preferred by annotators.
  % \vspace{-0.2cm}
\end{itemize}
Our code and dataset splits are available at \mbox{\url{https://github.com/tomhosking/hiro}}.

\section{Related Work}
\label{sec:relatedwork}

\todo{make this a delta from hercules}


In \Cref{ch:hercules} we proposed a hybrid method that represents sentences from reviews as paths through a learned discrete hierarchy, then generates output sentences based on frequent paths through this hierarchy \citet{hosking-etal-2023-attributable}. While \textsc{Hercules} is attributable and scalable, the highly compressed bottleneck leads to frequent hallucination and generic output with poor coherence.

\paragraph{Opinion Summarization with LLMs}

% Prior approaches to generating summaries of reviews broadly fall into two categories. \textit{Extractive} methods generate summaries by selecting representative sentences from input reviews to use as the summary \citep{lexrank,angelidis-etal-2021-extractive,basu-roy-chowdhury-etal-2022-unsupervised}. These types of approach are scalable and inherently attributable, but result in summaries that are overly detailed and not coherent. \textit{Abstractive} methods `read' input reviews and generate novel language to use as the summary  \citep{brazinskas-etal-2020-unsupervised,iso-etal-2021-convex-aggregation}. The resulting summaries are more fluent and coherent, but most prior abstractive methods are only able to consider a limited number of input reviews, whether because of combinatoric complexity or a maximum input length.



% \citet{cattan-etal-2023-key} proposed using Key Point Analysis to generate summaries, but their approach requires labelled examples of key points, which may not be available in every domain.

\citet{louis-maynez-2023-opinesum} use a Natural Language Inference (NLI) model to construct `silver standard' summaries to use as training data for fine-tuning a pretrained language model \cite[T5,][]{t5}. However, their approach is computationally very expensive, calculating over 1B pairwise entailment relations between sentences in the training data, before fine-tuning a LLM. By contrast, HIRO uses a lightweight indexing encoder, combined with an off-the-shelf LLM that is prompted in a zero-shot manner.

Prompted Opinion Summarization with GPT-3.5 \citep{bhaskar-etal-2023-prompted} - only aspect specific, and requires a lot of calls to closed source models \todo{expand}

% \paragraph{Structured Encodings and Indexes}

% Prior work has investigated how to learn representations of data with richer structure and interpretability. \citet{DBLP:journals/corr/VendrovKFU15} propose learning an embedding space where the ordering of two pairs of samples could be inferred from their relative positions, but their method requires supervision of the correct ordering. \citet{opper-etal-2023-strae} describe a method for learning embeddings that explicitly include structural information, but they focus on representing structures, rather than on learning an ordering within the embedding space itself. \citet{10.1145/3539618.3591651} learn a tree-based index for passage retrieval concurrently with the dense embedding space, showing that this leads to improved retrieval performance. However, they focus on retrieving passages relevant to a query, rather than aggregating opinions.

\citet{sarthi2024raptor} \todo{add this}

\paragraph{Content Selection}

The idea of first selecting relevant parts of an input before generating output has been well studied \cite[][\textit{inter alia}]{kedzie-etal-2018-content,DBLP:conf/aaai/Puduppully0L19,amplayo2021unsupervised,narayan-etal-2023-conditional}, and has been shown to be very effective when used in conjunction with LLMs in the form of retrieval-augmented generation \cite[RAG,][]{rag}. \citet{xu2023retrieval} found that retrieval augmentation is beneficial even when using models that can accept long inputs.

\paragraph{Evaluation of Summaries}

Automatic evaluation of generated summaries is extremely challenging. Prior work has shown that ROUGE  \citep{lin-2004-rouge} scores correlate poorly with human assessments of summary quality \citep{shen2023opinsummeval,clark-etal-2023-seahorse,aharoni-etal-2023-multilingual}. Some datasets are created automatically, with references that are not directly based on the input reviews \citep{brazinskas-etal-2021-learning}. Modern summarization system outputs are now often preferred to human-written references \citep{goyal2022zeroshotnews,bhaskar-etal-2023-prompted}.

% \citet{shen2023opinsummeval} compared a range of automatic metrics to human judgements, but their experiments were limited to datasets involving small numbers of reviews, with the metric most highly correlated to human judgements having a context window of only 1024 tokens. 

SummaC \citep{laban-etal-2022-summac} is a \textit{reference-free} metric that uses an NLI model to evaluate the degree of support between a summary and the input documents, but it overly rewards trivial statements; using the obvious statement ``The hotel was a building'' as a summary for every entity achieves a near-perfect SummaC score of 99.9\% on \textsc{Space}, a dataset of hotel reviews \citep{angelidis-etal-2021-extractive}.

\citet{prevalence} propose a metric that uses a NLI model to evaluate \textit{prevalence}, i.e. how many input reviews contain supporting evidence for each sentence in a summary, and explicitly penalizes trivial or redundant output. However, we found it has a similar failure mode to SummaC, with the statement ``The rooms are clean and comfortable'' achieving a prevalence score of 72\% on \textsc{Space}. We propose a modification to prevalence in \Cref{sec:part3_autoeval} that penalizes overly generic summaries.

% Although considered to be the gold standard, human evaluation is also highly challenging; results may be biased by confounders \citep{10.1162/coli_a_00508,hosking2023human} and it is not feasible for annotators to read hundreds of reviews before rating a summary.


% Maybe:
% Synthesize, if you do not have: Effective Synthetic Dataset Creation Strategies for Self-Supervised Opinion Summarization in E-commerce - only OpoSum/Amazon/Flipkart (8-10 reviews each)

% Large-Scale and Multi-Perspective Opinion Summarization with Diverse Review Subsets
% https://arxiv.org/pdf/2310.13340.pdf
% RT and AmaSum

% To leave out:
% Unsupervised Opinion Summarization Using Approximate Geodesics (old and copied QT)

% Simple Yet Effective Synthetic Dataset Construction for
% Unsupervised Opinion Summarization (only aspect specific? why)

% Aspect-aware Unsupervised Extractive Opinion Summarization (essential just QT)

% TransSum: Translating Aspect and Sentiment Embeddings for Self-Supervised Opinion Summarization - no code, only Yelp/Amazon/RT


\begin{figure}[]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/4-hiro/PipelineDiagram.pdf}  
    % \vspace{-0.2cm}
    \caption{HIRO uses three modules to generate summaries of customer reviews. First, we use our encoder to \textbf{index} all sentences from input review into a learned hierarchy. Then we identify paths within this index that occur frequently, and \textbf{retrieve} the corresponding clusters of sentences. Finally, we pass these clusters to an LLM to \textbf{generate} an output summary.}
    % \vspace{-0.2cm}
    \label{fig:hiro:pipeline}
    % \vspace{-0cm}
\end{figure}

\section{Overview}

Let $\mathcal{R}_e$ be a set of reviews about an entity $e \in \mathcal{E}$, where each review $\mathbf{R} \in \mathcal{R}_e$ is composed of a number of sentences $\mathbf{x}$. The goal is to generate a textual summary that includes the most informative opinions from $\mathcal{R}_e$, while abstracting away the details specific to any one review.

HIRO generates summaries following a modular approach, depicted in \Cref{fig:hiro:pipeline}. We learn an index structure that maps each sentence $\mathbf{x}$ from the input reviews to a path $q_{1:D}$ through a discrete hierarchy. We choose a hierarchical representation so that sentences are grouped at a useful level of abstraction; the upper levels of the hierarchy should partition sentences by topic, while the lowest levels should group together sentences with equivalent meaning.

At inference time, we encode all sentences from the reviews, then identify the paths or \textit{subpaths} $q_{1:d}$ within the index that are particularly \textit{popular}, and retrieve the corresponding sentences. This selection process is query-free, instead relying on properties of the hierarchical index to determine the frequency of different opinions. By indexing sentences hierarchically according to their semantics, we can easily identify opinions or topics that occur frequently by simply counting their occurrence in the index.

Finally, we generate a summary by passing the retrieved clusters of sentences as input to a LLM. This \textit{retrieval-augmented} usage of LLMs allows us to benefit from the fluency and coherence of LLMs, while retaining the attributability and scalability of extractive opinion summarization methods. 

We now detail the three modules that comprise HIRO, evaluating each of them in turn to confirm their efficacy compared to previous methods.


\section{Learning a Hierarchical Indexing}
\label{sec:part1}


Our goal is to learn an encoding space where sentences with similar meanings are grouped together. The space should be \textit{discretised} so that frequent opinions can be easily identified by counting the membership of each part of the index, and it should be \textit{hierarchical} so that opinions may be aggregated at an appropriate level of granularity, rather than by details or phrasings specific to a particular review. Finally, the encoding space should be structured semantically, to enable accurate aggregation of opinions; sentences with equivalent meaning should clearly be indexed to the same point in the hierarchy, while sentences that are topically related but not equivalent should be grouped together at a higher level.

% Shallow levels of the hierarchy should represent high level topics, while lower levels should group together sentences with very similar meanings, but potentially different surface forms.  

We base our encoder on HRQ-VAE \Cref{ch:bottleneck}. HRQ-VAE uses an encoder-decoder architecture with a discrete hierarchical bottleneck to generate summaries. It is trained as a denoising autoencoder, and therefore needs to learn a representation that is both compressed enough to enable aggregation, but also expressive enough for the decoder to be able to generate meaningful output. These factors are in direct competition, with the compressed bottleneck leading to output that is generic and contains hallucinations. By contrast, HIRO uses an external LLM as the `decoder', allowing us to focus on learning a representation that is useful for identifying informative opinions. 

% We hypothesize that this separation of concerns will allow for more control over the representation space, leading to an index that is more semantically distributed. 
% \todo{say here that we want a global arrangement of encoding space?} \citep{sherborne-etal-2023-optimal}
% \citep{JMLR:v11:radovanovic10a} - hubness


\subsection{Method}


The HIRO encoder module maps a single sentence $\mathbf{x}$ to a path $q_{1:D}$ through a discrete hierarchy, using the residual vector quantisation technique introduced in \Cref{ch:bottleneck} \citep{rvq,10.1109/TASLP.2021.3129994,hosking-etal-2023-attributable}. 

First, we use a Transformer encoder followed by attention pooling \citep{Vaswani2017,liu-lapata-2019-hierarchical} to map a sequence of tokens $\mathbf{x}$ to a single dense embedding $\mathbf{z} \in \mathbb{R}^{\mathbb{D}}$. Then, we decompose $\mathbf{z}$ into a path through a latent discrete hierarchy $q_{1:D}$, where $q_d \in \{1, \ldots, K\}$ are discrete `codes' at each level $d$. Briefly, we induce a distribution over codes at each level~$p(q_d)$, parameterised by a softmax with scores~$s_d$ given by the Euclidean distance from learned codebook embeddings to the residual error between the input and the cumulative embedding from all previous levels, 
\begin{align}
% \vspace{-.2cm}
\hspace{-0.25cm} s_d(q) = - \left( \left[\mathbf{z} - \sum\limits_{d'=1}^{d-1} \mathbf{C}_{d'}(q_{d'}) \right ] - \mathbf{C}_d(q)  \right ) ^2\hspace{-0.25cm} ,
% \vspace{-.2cm}
\end{align}
where $\textbf{C}_d \in \mathbb{R}^{K \times \mathbb{D}}$ is a codebook which maps each discrete code to a continuous embedding $\textbf{C}_d(q_d) \in \mathbb{R}^{\mathbb{D}}$. During training, we use the Gumbel reparameterisation
\citep{jang2016categorical,maddison2017concrete,sonderby2017continuous}
to sample from the distribution~$p(q_d)$. During inference, we set $q_d = \argmax s_d$.

Since our goal is to learn a representation where semantically similar sentences are grouped together, we use a training objective that explicitly induces this arrangement in encoding space. We train the encoder with a contrastive learning objective, bringing representations of semantically similar sentences (i.e., positive pairs) together, and pushing dissimilar ones apart. 

For each sentence in the training data, we construct positive pairs of semantically related sentences~$\mathbf{x},\mathbf{x}_+$ as follows: given a random `query' sentence $\mathbf{x}$ from the training data, we identify possible candidate `targets' based on tf-idf similarity; then, we check whether each candidate is entailed by the query using an NLI model \cite[DeBERTa v3, trained on Debiased NLI;][]{he2021debertav3,wu-etal-2022-generating}, and use the sentences which are labelled as entailed as positive targets~$\mathbf{x}_+$. An example is shown in \Cref{fig:trainingdata}. We do not use any `hard' negatives; instead, during training we calculate the pairwise tf-idf similarity between all samples in a batch, and include only those samples with similarity below a threshold of $0.3$ as negatives $\mathbf{X}_{-}$. This prevents `false negatives' being wrongly forced apart, and allows sentences that are topically related but not strictly equivalent to remain in the same high-level grouping within the index.

\begin{figure}[]
    \centering
    \includegraphics[width=0.58\textwidth]{figures/4-hiro/DataExample.pdf}  

    % \vspace{-.2cm}
    \caption{An example of the process for constructing the positive pairs used to train our model. Given a query sentence, we first use tf-idf to identify possible candidates from the training data, keeping only those sentences with similarity over a specified threshold. Then we check for entailment using an NLI model, and use any sentences labelled as `entailed' as positive targets. }
    % \vspace{-.2cm}
    \label{fig:trainingdata}
    % \vspace{-0cm}
\end{figure}



We found that it was crucial to include sufficient exploration in the process of constructing positive pairs. The candidate sentences retrieved using tf-idf should be sufficiently similar that we are likely to find ones that are entailed, but not so similar that they only have minor lexical differences.



We use a modified version of the InfoNCE training objective \citep{infonce} designed to bring the representations of a query $\mathbf{x}$ closer to those of a positive target $\mathbf{x}_+$, while pushing them apart from negative samples $\mathbf{X}_{-}$,
\begin{align}
    \mathcal{L} =& - \rho(\mathbf{x},\mathbf{x}_+) \log f,\\f=&  \frac{\exp\big(s(\mathbf{x},\mathbf{x}_+)\big)}{ \exp\big(s(\mathbf{x},\mathbf{x}_+)\big) + \frac{\omega}{\vert\mathbf{X}_{-}\vert} \sum\limits_{\mathbf{x}_{-}\in \mathbf{X}_{-}} \exp\big(s(\mathbf{x},\mathbf{x}_{-})\big) }, \notag
\end{align} 
where $\rho(\mathbf{x},\mathbf{x}_+)$ is the tf-idf similarity between $\mathbf{x}$ and $\mathbf{x}_+$ that weights the \textit{confidence} of the positive pairs, inspired by MarginMSE \citep{hofstatter2021improving}, and $\omega$ is a constant that controls the strength of the negative examples. The similarity function $s(\cdot,\cdot)$ is given by the mean dot product between the embedding of all subpaths $q_{1:d}$ for $d\leq D$,
\begin{align}
    \hspace{-0.2cm}s(\mathbf{x},\mathbf{x}') = \frac{1}{D} \sum\limits_{d=1}^D \max\big(  \mathbf{C}(q_{1:d})^T \mathbf{C}(q'_{1:d}), 0\big),
\end{align}
where $\mathbf{C}(q_{1:d}) = \sum_d \mathbf{C}_d(q_{d})$ is the full embedding of path $q_{1:d}$. Intuitively, this brings together the representations of the positive pairs at each level in the hierarchy, while penalizing any overlap with the representations of negative examples.

The similarity is floored at zero, to prevent the model from being able to `game' the loss by pushing negative examples further and further apart. Although the positive pairs are selected based on a directional entailment label, we do not exploit this directionality in our training objective.


We employ the techniques proposed in \Cref{ch:bottleneck} to induce a hierarchical encoding space proposed, including depth dropout, initialization decay, and norm loss. We additionally include the entropy of the distribution over codes, $-\sum_{d,q_d}\log\big(p(q_{d})\big)$, as an additional term in the objective, to encourage exploration of the latent space during training. Although HIRO is not a true generative model, this term is analagous to the KL term found in the ELBO.






\subsection{Evaluation}

We now evaluate whether the combination of discrete hierarchical encoding and contrastive objective leads to a more semantically distributed representation than previous methods.





\paragraph{Experimental Setup}
\label{sec:part1_eval}

We experiment using \textsc{{Space}} \citep{angelidis-etal-2021-extractive}, which consists of hotel reviews from TripAdvisor with 100 reviews per entity, as well as reference summaries created by annotators. We encode all the review sentences from the \textsc{Space} validation set, then calculate both the \textit{purity} (the mean intra-cluster similarity) and \textit{colocation} (the mean inter-cluster similarity) for the clusters of sentences assigned to each subpath $q_{1:d}$ for $d\leq4$. Finally, we take the difference between the purity and colocation as an overall measure of the quality of the representation space. 


We compare to \textsc{Hercules} (\Cref{ch:hercules}), which trains a hierarchical encoder jointly with a decoder. We also compare to a baseline using recursive $k$-means over embeddings from a pretrained embeddings model \cite[MiniLM,][]{reimers-gurevych-2019-sentence}: we apply $k$-means to the embeddings, then calculate the residual errors between cluster centroids and embeddings, apply $k$-means to those errors, and repeat. All methods use the same number of clusters at each level ($k=12$).

\begin{figure}[]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/4-hiro/encoding_quality.pdf}  
    % \vspace{-0.2cm}
    \caption{Cluster quality by depth, as measured by the difference between cluster purity and colocation, according to NLI (solid line) and tf-idf (dashed line) similarity measures. HIRO learns a higher quality encoding space than comparison methods.}
    % \vspace{-0.2cm}
    \label{fig:encoding_eval}
    % \vspace{-0.2cm}
\end{figure}

\paragraph{Model Configuration} We use a 6 layer Transformer, with token embeddings initialized from BERT base \citep{devlin-etal-2019-bert}.\footnote{We experimented with using BERT as the encoder but found no significant improvement, since the discrete encoding is the main bottleneck in the model.} We set the codebook size $K = 12$, with the number of levels $D = 12$, based on development set performance. Other hyperparameters are given in \Cref{appx:hparams}. 


\paragraph{HIRO learns a higher quality encoding space} \todo{can we use this kind of "headings as findings" throughout the thesis?}
\Cref{fig:encoding_eval} shows the overall quality (using both NLI and tf-idf measures of similarity), indicating that HIRO learns a more semantically distributed space at all levels of depth than comparison approaches, according to both similarity measures. The separation between clusters increases with depth, confirming that the encoder learns a semantic hierarchy. We believe these results indicate that our method could potentially be used for more general purpose document retrieval \cite[similar to][]{10.1145/3539618.3591651}, which is beyond the scope of this paper.

\section{Retrieving Popular Opinions}

Recall that a good summary should include opinions that occur repeatedly in the input reviews, as well as opinions that differentiate the current entity from others. 
% The HIRO retrieval module exploits the properties of the hierarchical index to select informative clusters of sentences from input reviews.
In \Cref{sec:part1} we showed how the HIRO encoder maps a single sentence $\mathbf{x}$ to a path $q_{1:D}$. We now exploit the discrete, hierarchical nature of the representation space to index a large number of review sentences, then identify informative sentences to use to generate a summary. We hypothesize that our content selection method leads to clusters that better represent the balance of opinions in the input reviews.

\subsection{Method}

For each review $\mathbf{R} \in \mathcal{R}_e$ about an entity $e \in \mathcal{E}$, we separately encode each sentence within the review to its path $q_{1:D}$, giving an indexed review $\mathbf{Q}(\mathbf{R})$.


Our content selection method identifies the parts of the hierarchy that are particularly popular for each entity, and extracts the corresponding clusters of sentences. This process is query-free; instead, we assign each subpath in the hierarchy $q_{1:d}$ a score based on its popularity within the indexed input reviews, and `retrieve' all sentences that were mapped to the $k$ highest-scoring subpaths.



Our scoring function is inspired by tf-idf \citep{tfidf}, which is designed to measure the importance of a particular term with respect to a set of baseline documents. We define the \textit{term popularity} $\tp(q_{1:d}, e)$ of a path as the fraction of indexed reviews for entity $e$ which contain the subpath $q_{1:d}$, 
\begin{align}
    \tp(q_{1:d}, e) =& \frac{1}{ |\mathcal{R}_e| }\sum_{\textbf{R} \in \mathcal{R}_e} \mathbb{I}\big(q_{1:d} \in \mathbf{Q}(\textbf{R}) \big) ,
    \label{eq:tp}
\end{align}
where $\mathbb{I}$ is the indicator function.
We define the \textit{inverse baseline popularity} $\ibp$ as the reciprocal of the mean term popularity across \textit{all entities} $\mathcal{E}$, 
\begin{align}
    \ibp(q_{1:d}) =& \biggl( \frac{\alpha + \sum_{e \in \mathcal{E}} \tp(q_{1:d}, e)}{\alpha + |\mathcal{E}|} \biggr)^{-1} ,
    \label{eq:ibp}
\end{align}
where the smoothing constant $\alpha$ allows us to  balance between absolute and comparative popularity. The overall score is then
\begin{align}
    \text{score}(q_{1:d}, e) =& \tp(q_{1:d}, e) \times \ibp(q_{1:d}) .
    % \label{eq:scoring}
\end{align} 
Intuitively, the score represents the relative popularity within the current entity of a path $q_{1:d}$ compared to all entities in the dataset.

Our scoring scheme conveniently accounts for the fact that short paths are more common;\footnote{The presence of a path $q_{1:D}$ for a review also implies the presence of all subpaths $q_{1:d}, d<D$.} short paths will also have a higher baseline popularity, leading to an overall score that is effectively normalized for the depth of the subpath.

After retrieving the clusters of sentences corresponding to the top-$k$ highest scoring subpaths, we filter out sentences with very low lexical similarity to other cluster members, and combine any clusters of sentences with high lexical overlap.

% The HIRO index is constructed based on entailment relations, and therefore places sentences about similar topics, but with different sentiment, in different parts of the hierarchy. We found that in some cases where opinions about a particular aspect of the entity were mixed, our method would retrieve distinct clusters with the positive and negative opinions separated out. We therefore merge together any selected clusters of sentences which have high lexical similarity to other clusters, allowing the generation module to reflect the mixed sentiments about a given aspect


\subsection{Evaluation}

We evaluate whether our method successfully selects clusters of sentences containing informative opinions, using reviews from \textsc{Space}, as in \Cref{sec:part1_eval}. First, we measure the overlap between retrieved clusters and \textit{oracle clusters} constructed by selecting sentences with high overlap to the reference summaries,\footnote{\textsc{Space} includes multiple reference summaries for each entity; we randomly select one when determining the oracle clusters.} using the Adjusted Rand Index \cite[ARI,][]{ari}. Second, we evaluate the average \textit{prevalence} \citep{prevalence} of sentences in retrieved clusters, which uses a NLI model \cite[ALBERT, trained on VitC;][]{albert,schuster-etal-2021-get} to evaluate how many input reviews support each retrieved sentence. 

We compare HIRO to the clusters extracted by \textsc{Hercules} \citep{hosking-etal-2023-attributable}, and the oracle upper bound. As a baseline, we apply $k$-means to MiniLM embeddings \citep{reimers-gurevych-2019-sentence}, then extract the 25 sentences whose embeddings are closest to each centroid. For HIRO, we select the top $k=8$ subpaths for each entity, and set the smoothing constant $\alpha=6$. 

\paragraph{HIRO selects higher prevalence sentences}

\Cref{tab:cluster_eval} confirms that HIRO retrieves clusters that more closely match the oracle clusters, and contain opinions that are more prevalent in the input reviews compared to prior work. The oracle ARI score is less than 1 because some sentences appear multiple times in different clusters.

\begin{table}[]
    \centering
    \small
    \begin{tabular}{l|rr}
    \toprule
        \textbf{System} & \textbf{Prevalence} & \textbf{ARI} \\
        \midrule\midrule
        $k$-means & 38.1 & 0.59 \\
        \textsc{Hercules} & 32.3 & 0.50 \\
        HIRO & \textbf{46.5} & \textbf{0.69} \\
        \midrule
        % (Oracle) & 49.7 & 0.87 \\
        (Oracle) & 48.1 & 0.73 \\
        \bottomrule
    \end{tabular}
    % \vspace{-0.2cm}
    \caption{Evaluation of our cluster selection method, compared to a range of baseline approaches. HIRO selects clusters of sentences that more closely match the references and contain more prevalent opinions.}
    % \vspace{-0.2cm}
    \label{tab:cluster_eval}
\end{table}


\section{Generating Coherent Summaries}

Given the retrieved clusters of sentences for each entity, we want to generate a coherent and fluent textual summary. LLMs are well suited to this constrained rewriting task, and we leverage the zero-shot abilities of instruction-tuned models to map clusters of sentences to a readable summary.

\subsection{Method}

We generate a summary from the retrieved clusters in three ways, with varying trade-offs between coherence and attributability, depicted in \Cref{fig:hiro:variants}.

\paragraph{HIRO\textsubscript{ext}} We generate \textit{extractive} summaries by selecting the centroid of each cluster; we compute all pairwise ROUGE-2 scores between sentences in each cluster, and choose the sentence with highest average similarity to other cluster members. This approach is fully attributable, since each summary sentence is extracted verbatim from a review.

\paragraph{HIRO\textsubscript{sent}} We generate summaries one sentence at a time by passing the contents of a single cluster as input to an instruction-tuned LLM with a simple prompt that requests a single sentence that summarizes the main points. This leads to more fluent output that is still attributable, since each output sentence has an associated cluster of evidential sentences used to generate it.

\paragraph{HIRO\textsubscript{doc}} We generate summaries as a single document, by passing the sentences from all retrieved clusters for an entity to the LLM in one go. This gives summaries that are more coherent and less redundant, since the LLM has control over the whole summary. However, it is not possible to identify which cluster was used to generate each part of the summary, so the attributability is less granular. 

The ideal balance between coherence and attributability is likely to vary by application.

\begin{figure}[]
    \centering
    \begin{subfigure}{0.69\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figures/4-hiro/HiroVariantsExtractive.pdf}
        \caption{HIRO\textsubscript{ext}}
        \label{fig:hiro:variants:ext}
    \end{subfigure}%
    \vspace{1em}
    \vspace{1em}
    
    \begin{subfigure}{0.69\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figures/4-hiro/HiroVariantsSent.pdf}
        \caption{HIRO\textsubscript{sent}}
        \label{fig:hiro:variants:sent}
    \end{subfigure}%
    \vspace{1em}
    \vspace{1em}
    
    \begin{subfigure}{0.69\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figures/4-hiro/HiroVariantsDoc.pdf}
        \caption{HIRO\textsubscript{doc}}
        \label{fig:hiro:variants:doc}
    \end{subfigure}
    \caption{Diagrams depicting the three variants of HIRO: extractive, sentence-wise, and document-level.}
    \label{fig:hiro:variants}
\end{figure}

\paragraph{Experimental Setup}

For the sentence-wise and document variants, we use Mistral 7B Instruct v0.2 to generate summaries from retrieved clusters. The LLM is queried in a zero-shot manner, and the prompts used are given in \Cref{appx:prompts}. We sample with a temperature of $0.7$, and report the mean and standard deviation scores based on 3 samples.

\subsection{Automatic Evaluation}
\label{sec:part3_autoeval}

Human evaluation is the gold standard (\Cref{sec:part3_humeval}), but automatic metrics remain useful for model development. ROUGE scores are no longer reliable and SummaC overly rewards generic summaries (\Cref{sec:relatedwork}), but we nonetheless report them for consistency with prior work. \citet{prevalence} propose a \textit{prevalence} metric, that uses an NLI model to determine how many input reviews contain supporting evidence for each sentence in the summary, but this suffers from a failure mode that overly rewards generic statements. A good summary should include common opinions, but should also help a user to differentiate between multiple entities. 


% \paragraph{Specificity Adjusted Prevalence}

To counteract this pathology, we propose a modified version of prevalence, that explicitly penalizes generic summaries. First, we define the \textit{genericness} of a summary as the average number of summaries from \textit{other entities} that support each sentence in a given summary, as measured by an NLI model \cite[ALBERT, trained on VitC;][]{albert,schuster-etal-2021-get}. Then, we define the Specificity Adjusted Prevalence score (SAP) as 
\begin{equation}
\texttt{SAP} = \texttt{prevalence} - \alpha~\texttt{genericness},    
\end{equation}
where $\alpha$ is a constant that controls the balance between absolute prevalence and specificity. In practice, the ideal summary is unlikely to be entirely unique and a user may want to allow some degree of overlap between generated summaries. We report the prevalence and genericness, as well as the combined SAP with $\alpha=0.5$. We also plot Specificity against Prevalence in \Cref{fig:spec_vs_prev}, with HIRO clearly exhibiting the best tradeoff between the two factors.

% \newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}}

\begin{table*}[]
    \centering
    \small
    \begin{tabular}{@{~}l@{~~}l@{~}||@{~}r@{~}r@{~}|@{~}r@{~}r@{~}r@{~}|@{~}r@{~}r@{~}}
    \toprule
     & & \multicolumn{7}{c}{\textbf{\textsc{Space}}} \\
    & \textbf{System} & {R-2} $\uparrow$  & {{R-L}} $\uparrow$  & {Prev.} $\uparrow$ & {Gen.} $\downarrow$ & {SAP} $\uparrow$ &  {SC\textsubscript{ins}} $\uparrow$ & {SC\textsubscript{refs}} $\uparrow$  \\
\midrule \midrule


\multirow{7}{*}{\rotatebox{90}{\textit{Extractive}}}  

   % \midrule
 & Random &  6.2\fshiro &  17.1\fshiro &  18.0\fshiro &  12.5\fshiro &  11.8\fshiro &  51.5\fshiro &  26.0\fshiro  \\ 
 & $k$-means &  9.5\fshiro &  19.8\fshiro &  27.9\fshiro &  25.0\fshiro &  15.4\fshiro &  72.7\fshiro &  31.0\fshiro  \\ 
 & LexRank &  5.9\fshiro &  16.4\fshiro &  18.2\fshiro &  \textbf{4.4}\fshiro &  16.0\fshiro &  54.4\fshiro &  22.6\fshiro  \\ 
 & QT &  10.3\fshiro &  21.5\fshiro &  25.0\fshiro &  23.3\fshiro &  13.3\fshiro &  \textbf{93.8}\fshiro &  41.2\fshiro  \\ 
 & SemAE &  11.1\fshiro &  23.5\fshiro &  29.2\fshiro &  17.1\fshiro &  20.7\fshiro &  65.9\fshiro &  27.9\fshiro  \\ 
 & \textsc{Hercules}\textsubscript{ext} &  \textbf{13.2}\fshiro &  \textbf{24.4}\fshiro &  30.2\fshiro &  25.2\fshiro &  17.6\fshiro &  89.0\fshiro &  \textbf{44.0}\fshiro  \\ 
 & HIRO\textsubscript{ext} &  11.7\fshiro &  22.1\fshiro &  \textbf{36.3}\fshiro &  20.5\fshiro &  \textbf{26.1}\fshiro &  82.1\fshiro &  37.4\fshiro  \\ 

 \midrule
 \multirow{9}{*}{\rotatebox{90}{\textit{Abstractive}}}  
   & CopyCat &  12.1\fshiro &  22.9\fshiro &  \textbf{48.3}\fshiro &  70.9\fshiro &  12.9\fshiro &  77.2\fshiro &  37.3\fshiro  \\ 
 & Mistral 7B &  5.3{\tiny$\pm$0.1}  &  19.6{\tiny$\pm$0.4}  &  41.3{\tiny$\pm$1.3}  &  34.3{\tiny$\pm$3.3}  &  24.2{\tiny$\pm$0.8}  &  52.5{\tiny$\pm$1.5}  &  24.6{\tiny$\pm$0.5}   \\ 
 & Llama 2 7B &  4.4{\tiny$\pm$0.2}  &  17.6{\tiny$\pm$0.1}  &  32.6{\tiny$\pm$3.0}  &  25.7{\tiny$\pm$3.7}  &  19.7{\tiny$\pm$2.3}  &  58.3{\tiny$\pm$1.0}  &  24.8{\tiny$\pm$0.3}   \\ 
 & Llama 2 13B &  5.5{\tiny$\pm$0.3}  &  18.7{\tiny$\pm$0.2}  &  29.5{\tiny$\pm$0.9}  &  27.4{\tiny$\pm$0.6}  &  15.8{\tiny$\pm$0.6}  &  54.9{\tiny$\pm$1.3}  &  24.5{\tiny$\pm$0.2}   \\ 
 & BiMeanVAE &  13.7\fshiro &  27.1\fshiro &  45.0\fshiro &  61.4\fshiro &  14.2\fshiro &  75.1\fshiro &  36.2\fshiro  \\ 
 & COOP &  14.2\fshiro &  \textbf{27.2}\fshiro &  46.1\fshiro &  63.2\fshiro &  14.5\fshiro &  77.5\fshiro &  39.4\fshiro  \\ 
 & \textsc{Hercules}\textsubscript{abs} &  \textbf{14.8}\fshiro &  \textbf{27.2}\fshiro &  32.2\fshiro &  36.1\fshiro &  14.1\fshiro &  \textbf{95.1}\fshiro &  \textbf{60.2}\fshiro  \\ 
 & HIRO\textsubscript{sent} Mistral 7B &  4.5{\tiny$\pm$0.1}  &  18.2{\tiny$\pm$0.0}  &  36.4{\tiny$\pm$0.9}  &  \textbf{20.2}{\tiny$\pm$0.4}  &  26.3{\tiny$\pm$1.0}  &  57.1{\tiny$\pm$0.3}  &  24.7{\tiny$\pm$0.1}   \\ 
 & HIRO\textsubscript{doc} Mistral 7B &  7.0{\tiny$\pm$0.2}  &  20.5{\tiny$\pm$0.3}  &  44.0{\tiny$\pm$3.0}  &  28.8{\tiny$\pm$2.1}  &  \textbf{29.6}{\tiny$\pm$2.1}  &  55.0{\tiny$\pm$0.5}  &  24.2{\tiny$\pm$0.6}   \\ 
 \midrule
 & (References) &  74.4\fshiro &  76.7\fshiro &  44.3\fshiro &  50.2\fshiro &  19.2\fshiro &  61.3\fshiro &  91.3\fshiro  \\ 
 & (Oracle) &  45.0\fshiro &  53.3\fshiro &  41.0\fshiro &  38.5\fshiro &  21.7\fshiro &  69.3\fshiro &  69.6\fshiro  \\ 
    \bottomrule



    \end{tabular}
% \vspace*{-.2cm}
    \caption{Results for automatic evaluation of summary generation, on Space. R-2 and R-L represent ROUGE-2/L F1 scores, and SC\textsubscript{ins} and SC\textsubscript{refs} refer to the SummaC scores against the input reviews and reference summaries respectively. Prev. refers to Prevalence, Gen. refers to Genericness, and SAP refers to Specificity-Adjusted Prevalence. We consider SAP to be our primary metric. The best scores for extractive and abstractive systems are shown in bold. Results for systems involving LLMs are based on 3 samples, with the mean and standard deviation shown. HIRO generates summaries with the best balance between prevalent opinions and specificity.}
     % \vspace*{-.2cm}
    \label{tab:hiro:automatic_general:space}
\end{table*}

\begin{table*}[]
    \centering
    \small
    \begin{tabular}{@{~}l@{~~}l@{~}||@{~}r@{~}r@{~}|@{~}r@{~}r@{~}r@{~}|@{~}r@{~}r@{~}}
    \toprule
     & & \multicolumn{7}{c}{\textbf{AmaSum}} \\
    & \textbf{System} & {R-2} $\uparrow$  & {{R-L}} $\uparrow$  & {Prev.} $\uparrow$ & {Gen.} $\downarrow$ & {SAP} $\uparrow$ &  {SC\textsubscript{ins}} $\uparrow$ & {SC\textsubscript{refs}} $\uparrow$  \\
\midrule \midrule


\multirow{7}{*}{\rotatebox{90}{\textit{Extractive}}}  

   % \midrule
 & Random &  1.0\fshiro &  9.5\fshiro &  16.3\fshiro &  8.0\fshiro &  12.3\fshiro &  59.2\fshiro &  22.4\fshiro  \\ 
  & $k$-means &  2.3\fshiro &  12.0\fshiro &  14.9\fshiro &  11.4\fshiro &  9.1\fshiro &  73.9\fshiro &  23.3\fshiro  \\ 

 & LexRank &  2.7\fshiro &  12.2\fshiro &  9.0\fshiro &  \textbf{3.0}\fshiro &  7.5\fshiro &  67.2\fshiro &  23.5\fshiro  \\ 
 & QT &  1.5\fshiro &  11.4\fshiro &  10.9\fshiro &  7.3\fshiro &  7.3\fshiro &  66.2\fshiro &  22.4\fshiro  \\ 
 & SemAE &  1.6\fshiro &  11.3\fshiro &  8.7\fshiro &  4.1\fshiro &  6.7\fshiro &  57.2\fshiro &  21.8\fshiro  \\ 
 & \textsc{Hercules}\textsubscript{ext} &  \textbf{3.0}\fshiro &  12.5\fshiro &  9.5\fshiro &  6.7\fshiro &  6.2\fshiro &  \textbf{84.0}\fshiro &  24.4\fshiro  \\ 
 & HIRO\textsubscript{ext} &  2.7\fshiro &  \textbf{12.6}\fshiro &  \textbf{19.4}\fshiro &  9.5\fshiro &  \textbf{14.6}\fshiro &  83.5\fshiro &  \textbf{24.7}\fshiro  \\

 \midrule
 \multirow{9}{*}{\rotatebox{90}{\textit{Abstractive}}}  
 & CopyCat &  1.5\fshiro &  11.2\fshiro &  15.8\fshiro &  21.0\fshiro &  5.3\fshiro &  63.1\fshiro &  23.0\fshiro  \\ 
 & Mistral 7B &  1.9{\tiny$\pm$0.0}  &  12.6{\tiny$\pm$0.0}  &  17.3{\tiny$\pm$0.2}  &  17.6{\tiny$\pm$0.4}  &  8.5{\tiny$\pm$0.2}  &  50.6{\tiny$\pm$0.2}  &  22.0{\tiny$\pm$0.0}   \\ 
 & Llama 2 7B &  1.5{\tiny$\pm$0.0}  &  11.5{\tiny$\pm$0.0}  &  17.7{\tiny$\pm$0.4}  &  17.6{\tiny$\pm$0.4}  &  8.9{\tiny$\pm$0.5}  &  58.6{\tiny$\pm$0.1}  &  22.6{\tiny$\pm$0.0}   \\ 
 & Llama 2 13B &  1.6{\tiny$\pm$0.1}  &  12.0{\tiny$\pm$0.1}  &  15.4{\tiny$\pm$0.2}  &  17.6{\tiny$\pm$0.2}  &  6.6{\tiny$\pm$0.3}  &  51.7{\tiny$\pm$0.3}  &  22.1{\tiny$\pm$0.0}   \\ 
 & BiMeanVAE &  2.0\fshiro &  12.5\fshiro &  14.7\fshiro &  24.1\fshiro &  2.7\fshiro &  52.5\fshiro &  21.8\fshiro  \\ 
 & COOP &  2.8\fshiro &  14.1\fshiro &  \textbf{18.8}\fshiro &  30.3\fshiro &  3.7\fshiro &  58.3\fshiro &  22.5\fshiro  \\ 
 & \textsc{Hercules}\textsubscript{abs} &  2.0\fshiro &  11.8\fshiro &  8.5\fshiro &  9.2\fshiro &  3.9\fshiro &  \textbf{82.7}\fshiro &  \textbf{25.2}\fshiro  \\ 
 & HIRO\textsubscript{sent} Mistral 7B &  3.5{\tiny$\pm$0.0}  &  14.1{\tiny$\pm$0.1}  &  14.6{\tiny$\pm$0.3}  &  \textbf{6.9}{\tiny$\pm$0.1}  &  \textbf{11.2}{\tiny$\pm$0.3}  &  53.8{\tiny$\pm$0.3}  &  22.7{\tiny$\pm$0.0}   \\ 
 & HIRO\textsubscript{doc} Mistral 7B &  \textbf{4.0}{\tiny$\pm$0.0}  &  \textbf{15.1}{\tiny$\pm$0.1}  &  15.3{\tiny$\pm$0.1}  &  9.4{\tiny$\pm$0.3}  &  10.6{\tiny$\pm$0.1}  &  46.8{\tiny$\pm$0.5}  &  21.9{\tiny$\pm$0.0}   \\ 
 \midrule
 & (References) &  83.4\fshiro &  85.3\fshiro &  9.3\fshiro &  7.0\fshiro &  5.8\fshiro &  66.2\fshiro &  86.4\fshiro  \\ 
 & (Oracle) &  14.4\fshiro &  26.0\fshiro &  12.3\fshiro &  9.0\fshiro &  7.8\fshiro &  76.3\fshiro &  26.4\fshiro  \\ 
    \bottomrule



    \end{tabular}
% \vspace*{-.2cm}
    \caption{Results for automatic evaluation of summary generation, on AmaSum.}
     % \vspace*{-.2cm}
    \label{tab:hiro:automatic_general:amasum}
\end{table*}


\begin{figure}[]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/4-hiro/specificity_vs_prevalence_space.pdf}
    \caption{A plot showing Specificity against Prevalence for all models evaluated, for Space. The ideal model would fall in the top-right corner of the plot. There is a clear tradeoff between the two - CopyCat generates summaries with high Prevalence scores, but low Specificity, and vice-versa for LexRank. In general, extractive systems (marked with an X) are more specific but less prevalent than abstractive systems (marked with a disc), since the summaries comprise complete sentences from input reviews. All three variants of HIRO offer the best tradeoff between the competing factors.}
    \label{fig:spec_vs_prev}
\end{figure}



\paragraph{Datasets} We evaluate summary generation using \textsc{Space} (\Cref{sec:part1_eval}), which includes multiple reference summaries created by human annotators for each entity. We also include \textbf{AmaSum} \citep{brazinskas-etal-2021-learning}, to evaluate summary generation on a wide range of categories of Amazon products, with an average of 560 reviews per entity. The reference summaries were collected from professional review websites, and therefore are not necessarily grounded in the input reviews. We use the same splits, based on four product categories, as released by \citet{hosking-etal-2023-attributable}. We found that it was not necessary to train HIRO on a single product domain, and so we report results for a single HIRO model trained on all four product categories.


\paragraph{Comparison Systems}
We select a \textbf{random review} from the inputs as a lower bound. 
% We also select the \textbf{centroid} of the set of reviews, according to ROUGE-2 F1 score. 
We include an extractive \textbf{oracle} as an upper bound, by selecting the input sentence with highest ROUGE-2 similarity to each reference sentence.\footnote{When multiple references are available, we select one at random.} For a \textbf{k-means} baseline, we run $k$-means on MiniLM sentence embeddings \citep{reimers-gurevych-2019-sentence}, then extract the nearest sentence to the cluster centroids. We set $k=8$ to match the average sentence length of the reference summaries.

\textbf{Lexrank} \citep{lexrank} is an unsupervised extractive method using graph-based centrality scoring of sentences.

\textbf{QT} \citep{angelidis-etal-2021-extractive} uses vector quantisation to map sentences to a discrete encoding space, then generates extractive summaries by selecting representative sentences from clusters.

\textbf{SemAE} \citep{basu-roy-chowdhury-etal-2022-unsupervised} is an extractive method that extends QT, relaxing the discretisation and encoding sentences as mixtures of learned embeddings.
% - meansum \citep{meansum}

\textbf{CopyCat} \citep{brazinskas-etal-2020-unsupervised} is an abstractive approach that models sentences as observations of latent variables representing entity opinions, trained in a `leave one out' manner.

\textbf{BiMeanVAE} and \textbf{COOP} \citep{iso-etal-2021-convex-aggregation} are abstractive methods that encode full reviews as continuous latent vectors using an autoencoder, and take the average (BiMeanVAE) or an optimised combination (COOP) of review encodings.

We compare to a recent open weight instruction-tuned \textbf{LLM}, specifically Mistral Instruct v0.2 7B \citep{jiang2023mistral}. To evaluate the effect of model size, we compare to Llama 2 Chat 7B and 13B \citep{touvron2023llama}, which are equivalent models apart from parameter count. The LLMs are prompted zero-shot using the prompt in \Cref{appx:prompts}, and sampled with temperature $0.7$. We report the mean and standard deviation scores based on 3 samples. In \Cref{ch:hercules} we compared to InstructGPT; however, commercial closed-weight models are not reproducible, since the precise model exposed by an API may change without notice. The model used in \Cref{ch:hercules} was no longer available at the time when the work in this chapter was performed. Additionally, commercial models incur substantial costs when performing inference. We therefore restrict our comparison to open-weight models and omit InstructGPT.

Most of the abstractive methods are not scalable and have upper limits on the number of input reviews. CopyCat and the LLMs have a maximum input sequence length, while COOP exhaustively searches over combinations of input reviews. We use 8 randomly selected reviews as input to CopyCat, COOP,  Llama 2, and Mistral 7B.


\paragraph{HIRO gives the best balance between prevalence and specificity}

The results in \Cref{tab:hiro:automatic_general:space,tab:hiro:automatic_general:amasum} show that HIRO achieves the highest SAP scores across both datasets, indicating that it generates summaries with the best balance between absolute prevalence and specificity. While CopyCat and COOP achieve the highest prevalence scores on \textsc{Space} and AmaSum respectively, they also display some of the highest genericness; qualitatively, the outputs are very similar to each other, and include no specific details about each entity. We give example outputs in Tables~\ref{tab:hiro:output} and \ref{tab:hiro:output2}, and an example of selected subpaths, sentence clusters and corresponding HIRO outputs in \Cref{tab:evidence_example}.


\paragraph{Increasing model size does not help} The SAP scores \textit{decrease} for the larger Llama 2 13B model compared to Llama 2 7B, indicating that increasing model size does not lead to improved performance. The short context window of current instruction-tuned LLMs limits the number of reviews they can take as input, preventing them from accurately reflecting the true distribution of opinions.

\paragraph{References are not the upper bound} 

While the oracle summaries score highly in terms of specificity-adjusted prevalence, some systems (including HIRO) outperform them. This indicates the difficulty with constructing reference summaries for entities with large numbers of reviews; it is not feasible for human annotators to reliably summarize such a large amount of information.



\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/4-hiro/path_dist.pdf}  
    % \vspace{-0.2cm}
    \caption{Distribution of selected subpaths by depth. A significant fraction of the extracted clusters come from paths deeper than the top level.}
    % \vspace{-0.2cm}
    \label{fig:path_dist}
    % \vspace{-0cm}
\end{figure}

\begin{table}[!t]
\small
    \centering
    \begin{tabular}{l|rr}
    \toprule
    \textbf{System} & \textbf{\% Partial} & \textbf{\% Majority} \\
    \midrule
        % \textsc{Hercules}\textsubscript{ext}  & 59.6 & 49.8 \\
       \textsc{Hercules}\textsubscript{abs}  & 85.4 & 27.6 \\
       % HIRO\textsubscript{ext} & 57.1 & \textbf{50.5} \\
        HIRO\textsubscript{sent} & 81.6 & 21.6 \\
        HIRO\textsubscript{doc} &  \textbf{91.8} & \textbf{28.4} \\
        \bottomrule
    \end{tabular}
    % \vspace{-0.2cm}
    \caption{Results for automatic evaluation of the evidence supplied by attributable systems, showing the percentage of summary sentences that have support from at least one sentence in the evidence set (partial support) and from at least half the sentences in the evidence (majority support). HIRO generates summaries that have strong partial support from the associated evidence sets, with improved majority support compared to \textsc{Hercules}.} 
    % \vspace{-0.2cm}
    \label{tab:attribution}
\end{table}


\begin{figure*}[]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/4-hiro/human_eval.pdf}  

    % \vspace{-.2cm}
    \caption{Results of our human evaluation. Crowdworkers were asked for pairwise preferences between generated summaries in terms of their Accuracy, Detail, and Coherence \& Fluency, as well as an overall preference. HIRO generates more coherent and detailed summaries that better represent the opinions in the input reviews than comparison systems, and are preferred by human annotators.}
    % \vspace{-.2cm}
    \label{fig:hiro:human_eval}
    % \vspace{-0cm}
\end{figure*}

\paragraph{HIRO is more attributable} 

To evaluate how faithful the generated summaries are to the retrieved sentence clusters or \textit{evidence sets}, we use an NLI model to determine how many sentences in each cluster either entail or are entailed by the corresponding sentence in the output summary, and take the mean. Considering both forward and backward entailment in this manner accounts for the different levels of granularity between the inputs and summary \citep{zhang-etal-2024-fine}; input reviews are likely to be more specific than summary sentences, but concise summary sentences are likely to contain multiple assertions, e.g. ``The food was good \textit{and} the rooms were clean''. HIRO\textsubscript{doc} does not align the evidence sets with each generated sentence, so we calculate the maximum support score over all sets for each summary sentence. Most abstractive systems are not attributable, and so we only compare with \textsc{Hercules}. \Cref{tab:attribution} shows the percentage of summary sentences that have support from at least \textit{one} sentence in the evidence (partial support) and from at least \textit{half} the sentences in the evidence (majority support). HIRO\textsubscript{doc} generates summaries that have strong partial support from the associated evidence sets, with improved majority support compared to \textsc{Hercules} despite also being significantly more detailed.



\paragraph{HIRO makes use of the hierarchy} We confirm that HIRO exploits the hierarchical nature of the representation space. \Cref{fig:path_dist} shows the distribution of selected subpath depths for both datasets, indicating that HIRO takes advantage of the hierarchy and selects clusters deeper than the top level. This is particularly true for AmaSum, where there is a wider range of product types, causing the selection process to search deeper in the tree.

\subsection{Human Evaluation}
\label{sec:part3_humeval}

We conduct a human evaluation to verify that HIRO generates summaries that are coherent and accurately reflect the opinions in the input reviews. We recruit crowdworkers through Prolific, and show them a set of 50 reviews, followed by two generated summaries. Using an interface based on Potato \citep{pei2022potato}, we solicit pairwise preferences along three dimensions, as well as an overall preference: 
\begin{itemize}
% \vspace{-0.3em}
% \setlength\itemsep{-0.3em}
    \item \textbf{Accuracy} ---  Which summary accurately reflects the balance of opinion in the  reviews?
    \item \textbf{Detail} --- Which summary includes more specific details?
    \item \textbf{Coherence} --- Which summary is easy to read and avoids contradictions?
    \item \textbf{Overall} --- Which summary do you think is better, overall?
    % \vspace{-0.3em}
\end{itemize}

The full instructions are reproduced in \Cref{appx:annotation}. We gather annotations for  10~entities each from the \textsc{Space} and AmaSum test sets, with 3~annotations for each. 

We compare HIRO\textsubscript{doc} to the top performing extractive and abstractive systems from \Cref{tab:hiro:automatic_general:space,tab:hiro:automatic_general:amasum}, SemAE and \textsc{Hercules}\textsubscript{abs}. HIRO\textsubscript{doc} uses Mistral 7B as the generator, so we also compare to Mistral 7B \textit{without} HIRO (i.e., prompted directly with reviews). Finally, we include a random review as a lower bound, and the references as an upper bound.

\paragraph{Humans prefer summaries generated by HIRO}

The results in \Cref{fig:hiro:human_eval} show that HIRO\textsubscript{doc} produces summaries that outperform comparison systems across all dimensions, producing summaries that coherently and accurately represent the opinions in the input reviews. Differences between HIRO\textsubscript{doc} and other systems are significant in all cases (using a one-way
ANOVA with post-hoc Tukey HSD test, $p<0.05$), except for coherence versus Mistral 7B. Both Mistral 7B and HIRO\textsubscript{doc} outperform the reference summaries, supporting findings from prior work \citep{bhaskar-etal-2023-prompted,hosking2023human}.



\begin{figure}[]
    \centering
    \includegraphics[width=0.55\textwidth]{figures/4-hiro/human_eval_hiro.pdf}  

    % \vspace{-.2cm}
    \caption{Results of a human evaluation comparing the three variants of HIRO: extractive, sentence-wise and document. Overall, annotators prefer the coherent of the document approach, but the sentence-wise variant generates more detailed summaries that are also more attributable. The preferred tradeoff between coherence and attribution will vary depending on the application.}
    % \vspace{-.2cm}
    \label{fig:hiro:human_eval_hiro}
    % \vspace{-0cm}
\end{figure}

\paragraph{Comparing HIRO variants} We run an additional human evaluation to evaluate the tradeoff between quality and attribution between the three HIRO variants, collecting annotations for 5 entities from each dataset from 3 annotators each. \Cref{fig:hiro:human_eval_hiro} shows that annotators prefer the output of HIRO\textsubscript{doc}, although the sentence-wise variant generates more detailed summaries. The preferred tradeoff between attribution and coherence will likely vary depending on the application.
    


% \subsection{Ablation Studies}

% - Different LLMs
% - remove components: no HRQ loss, no tfidf scores, no inbatch neg mask






% \paragraph{Example outputs}\todo{be clearer about what I'm trying to show - are these indicative of general perf?} We show some examples of output summaries from all three variants of HIRO in \Cref{tab:hiro:output}, alongside a summary generated by Mistral 7B. Although each sentence in the extractive output corresponds to some prevalent opinion from the input, it includes extraneous details that are more appropriately presented in the sentence-wise output. However, the one-shot variant produces summaries that are coherent while still reflecting the prevalence of opinions across all input reviews. The LLM output is also coherent and compelling, but is based on a small subset of the input reviews, and so is an unreliable representation of their contents.



% \setlength{\baselineskip}{0.5\baselineskip}
\begin{table*}[]
\renewcommand{\arraystretch}{1.0}

    \centering
    \small
    \begin{tabular}{m{2cm}| >{\setlength{\baselineskip}{0.5\baselineskip}}m{12cm} }
    \textbf{System} & \textbf{Output} \\
    \midrule\midrule
    % ix=20
\textit{Reference} & 
The staff were very welcoming and were always happy to help you with whatever was needed. The comfortably-sized rooms were very nice and clean, and the bathrooms were exceptionally clean and well equipped. Breakfast was continental and included in the price, offering baguettes, croissants, cereal, yogurts, etc.
 \\ 
 \midrule  
% \textit{Random \newline Review} & 
% A real parisienne experience. The hotel is a beautiful building and the location perfect. We walked everywhere and the local area is a delight with many bars and FRIENDLY restaurants. We are an older couple and went to Paris to get engaged - it was all perfect and the hotel's ambience added to the experience. Highly recommended if you want a small, local hotel as opposed to a large modern one. Many thanks - we would return and recommend you to friends. Margaret and David
%  \\ 
 % \midrule  
% \textit{SemAE} & 
% We were able to walk to all the tourists sights, except Montmarte and the Eiffel Tower.	The hotel staff was very friendly and helpful during our stay.	The staff is very friendly and helpful and the breakfast is a perfect start to the day.	The rooms was sufficent in size, the bed and pillows were very comfortable.	The ladies in the breakfast area were very friendly and courteous.	The bathroom was clean and the shower
%  \\ 
%  \midrule  
\textit{CopyCat} & 
We stayed at this hotel for 3 nights. The hotel was very clean and the staff very helpful. The location is perfect for exploring the city and the metro station is a short walk away. We will be back!
 \\ 
 \midrule  
% \textit{COOP} & 
% The hotel is in a great location, close to the metro and the metro. The staff were very friendly and helpful. The rooms were clean and comfortable, and the breakfast was very good. The hotel is in a great location, close to the Metro and the metro. The only downside is that the rooms are a little on the small side, but they are very clean and the staff is very friendly and helpful.
%  \\ 
%  \midrule  
\textit{\textsl{Hercules}\textsubscript{abs}} & 
The room was clean and comfortable. The staff was very friendly and helpful. walking distance to everything. The room was clean and comfortable. breakfast was good. The hotel is in a great location, just a few minutes walk from the train station. breakfast was fine. The room and bathroom were very clean. The staff spoke English and were very helpful. There is also a small restaurant on the ground floor.
 \\ 
 \midrule  
\textit{Mistral 7B} & 
The St. Christophe Hotel in Paris offers small, clean, and cozy rooms in a lively neighborhood near the Place Contrascarpe and Rue Mouffetard. The staff are helpful and friendly, and the location is convenient with easy access to metro stations and nearby restaurants. The hotel lacks air conditioning, so it may not be ideal during warm weather. Free Wi-Fi is available in the lobby. Overall, the St. Christophe Hotel is a charming and elegant choice for travelers to Paris.
 \\ 
 \midrule  
\textit{HIRO\textsubscript{ext}} & 
Nearby, and very close to 2 Metro stations. The hotel is 1 block to the Metro (line 7) between the North and South exits of the "place Monge" stop. The bathroom was clean and functional. The staff were friendly and helpful at all times. Breakfast was Plentiful-Cold cereal, great coffee, yogurt and a wonderful basket of Croissants, breads and Pastries. The shower excellent.
 \\ 
 \midrule  
\textit{HIRO\textsubscript{sent}} & 
The Hotel Saint Christophe is conveniently located near multiple metro stations. The Hotel Saint Christophe is centrally located near the Metro and restaurants in the Latin Quarter. The Hotel Saint Christophe offers clean, functional bathrooms in small rooms. The Hotel Saint Christophe's friendly and helpful staff provided excellent service. Breakfast offers cereal, yogurt, pastries, and hot beverages. Guests praised the Hotel Saint Christophe for its excellent showers.
 \\ 
 \midrule  
\textit{HIRO\textsubscript{doc}} & 
The Hotel Saint Christophe is centrally located in the Latin Quarter, close to multiple Metro stations and attractions such as Notre Dame and Jardin Luxembourg. Rooms are clean and adequate, though small, and breakfast offers a variety of options. The staff are friendly and helpful, making for a pleasant stay. The hotel is conveniently located near shops, restaurants, and markets. The bathrooms are clean and modern, though some may be smaller than expected for Paris.
    \end{tabular}
    % \vspace*{-.2cm}
    \caption{Examples of generated summaries for `Hotel Saint Christophe' in Paris, from \textsc{Space}. HIRO\textsubscript{doc} generates concise, informative and coherent summaries that accurately reflect the balance of opinions from input reviews. Mistral 7B prompted directly with reviews also generates coherent summaries, but these do not accurately reflect the overall balance of opinions. Previous abstractive systems, CopyCat and \textsc{Hercules}\textsubscript{abs}, generate generic summaries that lack detail.}
    % \vspace*{-.2cm}
    \label{tab:hiro:output}
\end{table*}

\begin{table*}[]
\renewcommand{\arraystretch}{1.2}
    \centering
    \small
    \begin{tabular}{m{2cm}|>{\setlength{\baselineskip}{0.5\baselineskip}}m{12cm}}
    \textbf{System} & \textbf{Output} \\
    \midrule\midrule
    % ix=18
\textit{Reference} & 
These headphones are your best option if you're looking for noise-cancelling earbuds, but they are pricey. Noise-cancelling earbuds. Available in black or white. Stay Hear tips keep earbuds in your ears while maximizing comfort. Impressive sound quality. Carrying case included. These are expensive for earbuds, so you should only buy them if you're going to use them often
 \\ 
 \midrule  
% \textit{Random \newline Review} & 
% Excellent. I’m comparing this to the Bose on ear headphones and this cancels noise better. I’m a frequent flyer and like to disappear during flights. This helps me get into another zone whether it’s listening to electro-house or watching the latest movies while flying. Highly recommend it!
%  \\ 
%  \midrule  
\textit{CopyCat} & 
So far so good. The only issue I have is that the volume is not as loud as my old one, but other than that I'm happy with this purchase.
 \\ 
 \midrule  
% \textit{COOP} & 
% These are the best ear buds out of the box. The sound quality is great, the bass is very good, and the noise cancelling feature is amazing. The only downside is that it doesn't have a USB-C port on the back of the device. It's not a big deal, but if you want to use it for work, you can't go wrong with this product.
%  \\ 
%  \midrule  
\textit{\textsl{Hercules}\textsubscript{abs}} & 
Love these Earbuds. These are great for listening to music. Noise cancelling works well. Long battery life. These are my favorite Headphones. The sound quality is very clear. The sound quality is great and the noise cancellation is good. Got this for my wife for Christmas. The sound quality is great and the Mic is clear. The Bass is a bit lacking. The ear pads are soft and comfortable. These Headphones are the best ever. The Headphones are very comfortable.
 \\ 
 \midrule  
\textit{Mistral 7B} & 
These earbuds have received positive reviews from users who travel frequently, find them a game changer, and have even convinced friends to buy them. Some users have purchased them for their children who are also satisfied. The earbuds have received five-star ratings from both the buyers and their sons. One user's wife loves them and uses them when the user snores at night. However, some users have noted that the noise-cancelling feature is not as effective as over-ear headphones.
 \\ 
 \midrule  
\textit{HIRO\textsubscript{ext}} & 
The noise cancelling is fantastic. These are the best Headphones I've ever owned. Well worth the money! The batteries last a long time and charge quickly. I have the over the ears pair and also these in the ears.
 \\ 
 \midrule  
\textit{HIRO\textsubscript{sent}} & 
The Bose QuietComfort 20 headphones offer exceptional noise cancellation and comfort. These Bose QuietComfort 20 headphones are exceptional, providing excellent noise cancellation and sound quality. These headphones are worth the investment due to their exceptional noise-cancelling capabilities. Battery lasts long for noise cancellation, charging quickly. Some users report over 10 hours usage. Some prefer Bose QuietComfort 20 earbuds for flights and noisy environments, others find them dizzying.
 \\ 
 \midrule  
\textit{HIRO\textsubscript{doc}} & 
The Bose QuietComfort 20 Acoustic Noise Cancelling Headphones are widely praised for their excellent noise cancellation capability, making them a popular choice for frequent flyers and those working in noisy environments. They are also praised for their comfort, sound quality, and long battery life. However, some customers have expressed concerns about the non-replaceable battery and the price. Overall, these headphones are considered a worthwhile investment for their impressive noise cancellation and sound quality.
    \end{tabular}
    % \vspace*{-.2cm}
    \caption{Examples of generated summaries for the `Bose QuietComfort 20' headphones, from AmaSum.}
    % \vspace*{-.2cm}
    \label{tab:hiro:output2}
\end{table*}

\begin{table*}[]
    
\renewcommand{\arraystretch}{0.8}
    \centering
    \small
    \begin{tabular}{m{2cm}|>{\setlength{\baselineskip}{0.5\baselineskip}}m{12cm}}
    \midrule\midrule
    \textit{$q_{1:d}$} & (6,2,10) \\
    \midrule
\multirow{16}{*}{\textit{Evidence}} & The pool area was very nice. \\ 
 & The staff was very Friendly and helpful. \\ 
 & the pool area was very enjoyable \\ 
 & The pool area is very nice. \\ 
 & The pool area is fantastic \\ 
 & The pool area was nice \\ 
 & the pool area is very attractive \\ 
 & The staff was so friendly and helpful. \\ 
 & The pool was nice \\ 
 & The staff was friendly and accommodating. \\ 
 & The pool was very nice and the lobby inviting \\ 
 & the staff was welcoming and helpful \\ 
 & The hotel staff was very friendly and accommodating. \\ 
 & Staff was friendly and helpful. \\ 
 & The pool area is very nice and large with several water features. \\ 
 & The staff was really great and helpful \\ 
\midrule
\textit{HIRO\textsubscript{sent}}  &  The pool area and friendly staff make this hotel a enjoyable stay. \\



    \midrule\midrule
    \textit{$q_{1:d}$} & (10, 8, 6) \\
    \midrule
\multirow{6}{*}{\textit{Evidence}} & 
Free parking is also available to the rear of the hotel. \\ 
 & Free parking in the hotel yard. \\ \ 
 & A big plus was the free parking and large selection for continental breakfast. \\ 
 & The free plentiful parking (some even under cover) is also one of the better features of the hotel. \\ 
 & It has free parking (a big deal in Key West), an awesome pool, and the best free continental breakfast I've ever seen. \\ 
 & Parking is free with some covered parking. \\
 
\midrule
\textit{HIRO\textsubscript{sent}} &  Free parking and continental breakfast are notable features of this hotel. \\

    \midrule\midrule
%     \textit{$q_{1:d}$} & (9,) \\
%     \midrule
% \multirow{9}{*}{\textit{Evidence}} & I was extremely disappointed in the rooms \\ 
%  & Only one mirror in the room. \\ 
%  & The rooms are loud. \\ 
%  & the rooms are awful \\ 
%  & the room was small and shabby \\ 
%  & we were a little disappointed because the room was a lot smaller than we expected \\ 
%  & Extremely disappointed in the room, although the help was very nice as was the outdoor area. \\ 
%  & i suspect we were in the older part of the hotel with a double room. \\ 
%  & Since the parking is directly under the rooms, it was Very loud espcially from 12-3 am. \\ 
% \midrule
% \textit{HIRO\textsubscript{sent}}   &  Rooms were small, loud, and in need of renovation with poor housekeeping. \\
% \midrule\midrule

% \textit{HIRO\textsubscript{doc}}   & The Fairfield Inn and Suites Key West received positive reviews for its friendly and helpful staff, attractive and nice pool area, and free parking. However, some guests were disappointed with the small and shabby rooms, lack of storage space, and noise from parking and adjacent rooms. The continental breakfast was also mentioned as a plus. \\
% \midrule\midrule
    
    \end{tabular}
    % \vspace*{-.2cm}
    \caption{Examples of selected subpaths $q_{1:d}$, the corresponding evidential clusters, the resulting HIRO\textsubscript{sent} output sentences, and the overall HIRO\textsubscript{doc} summary for the `Fairfield Inn', from \textsc{Space}. We show only two out of five input clusters, and a subset of all evidence sentences, due to space constraints.}
    % \vspace*{-.2cm}
    \label{tab:evidence_example}
\end{table*}

\section{Citations from LLMs}


\begin{table*}[]
\renewcommand{\arraystretch}{1.2}
    \centering
    \small
    \begin{tabular}{@{}c@{~~}r|>{\setlength{\baselineskip}{0.5\baselineskip}}m{9cm}}
    \toprule
    & \textbf{LLM} & \textbf{Output} \\
    \midrule\midrule
    
%     & Input prompt & Here are some groups of sentences taken from reviews of the Hotel Navona:

% [1]
% The breakfast was nothing to write home about.
% The breakfast was filling if nothing

% [2]
% The location is excellent.
% The location is central, walking distance to many interesting places in Rome.

% [3]
% The room was also small and dark.
% The rooms are ok, small bathrooms.

% [4]
% We walked back to the hotel because we were stuffed.
% We walked everywhere with our 5-year old from the hotel to include the coliseum, Pantheon, multiple churches (there are many in Rome!

% [5]
% The staff were very friendly and welcoming ( in particular Michele )
% The owner is friendly and accommodating as well as the staff

% [6]
% Our room even had 14th century paintings on the ceilings!
% Our room was exactly like the photo online

% [7]
% It was clean and air conditioned.
% The room was clean and very basic

% [8]
% The hotel has several floors and is a former 14th Century Palace.
% The hotel is on the first floor of an old building which smelt badly.

% In no more than 60 words, write a concise summary that includes the main points, citing which group contains the relevant information: \\
    % \midrule\midrule

    
     \multirow{1}{*}{\rotatebox{90}{\textit{Std prompt}}} & Mistral 7B & The Hotel Navona is centrally located in Rome, providing easy access to major attractions. The breakfast was described as average with small, basic rooms, some of which were noisy and dirty. Staff were consistently described as friendly and helpful, making up for any drawbacks. The hotel is in an old palazzo and retains much of its original charm. Some rooms feature 14th century paintings on the ceilings. Overall, the hotel's prime location and friendly staff make up for its minor drawbacks. \\
    \midrule
    \midrule
    
 \multirow{10}{*}{\rotatebox{90}{\textit{Citation prompt}}} & Mistral 7B & 
Group [1] and [3] primarily focus on the hotel's breakfast and room conditions, with complaints about the quality and size, as well as noise and cleanliness issues. [1] also mentions the location being average. Group [2] highlights the hotel's excellent location, which is central and convenient for accessing major Rome attractions. Group [5] emphasizes the friendly and helpful staff, with some mentioning specific staff members who went above and beyond. Group [6] consists of various comments about room assignments, including being fortunate to find the hotel, having rooms with historical features, and booking methods. Group [7] focuses on the hotel's cleanliness and basic accommodations, with some mentioning the small size and clean bathrooms. Group [8] touches on the hotel's history and cleanliness, with one comment mentioning a poor smell on the first floor.
 \\ 
 \cmidrule{2-3}
  
% \textit{Random \newline Review} & 
% Excellent. I’m comparing this to the Bose on ear headphones and this cancels noise better. I’m a frequent flyer and like to disappear during flights. This helps me get into another zone whether it’s listening to electro-house or watching the latest movies while flying. Highly recommend it!
%  \\ 
%  \midrule  
% \textit{COOP} & 
% These are the best ear buds out of the box. The sound quality is great, the bass is very good, and the noise cancelling feature is amazing. The only downside is that it doesn't have a USB-C port on the back of the device. It's not a big deal, but if you want to use it for work, you can't go wrong with this product.
%  \\ 
%  \midrule  
& LLama 3 8B Instruct & The hotel's location is a major strength, with many reviewers praising its central location and walking distance to major attractions (Group 2). However, some rooms are small and dark (Group 3), and the breakfast is unimpressive (Group 1). The staff is generally friendly and helpful (Group 4), and the hotel is clean and well-maintained (Group 7). The hotel's history and architecture are also notable, with some rooms featuring 14th-century paintings and frescoes (Group 6). \\
\cmidrule{2-3}
& Llama 3 70B Instruct & 
Hotel Navona's location is excellent, central, and within walking distance to major attractions (Group 2). The breakfast is average (Group 1). Rooms are small, but some are spacious and clean, with friendly staff (Groups 3, 5, and 7). The hotel has a rich history, being a former 14th-century palace (Group 8).
 \\ 
 \cmidrule{2-3}
& Cohere Command R+ (104B) & 
Reviewers praised the hotel's excellent location [2], with many attractions within walking distance. Opinions varied on room size and cleanliness [3], but the staff was friendly and helpful [5]. Breakfast was basic [1], and the hotel featured historical details [6,8]. Overall, the hotel was clean and air-conditioned [7].
 \\ 
 
 
 \bottomrule  

    \end{tabular}
    % \vspace*{-.2cm}
    \caption{Examples of summaries generated using HIRO clusters with a prompt that asks the model to include citations. All selected clusters are passed as input to the LLM, as in HIRO\textsubscript{doc}, but are now labelled with a cluster number. When prompted to include citations, Mistral 7B generates a summary one cluster at a time, which is overly long and much less coherent than Mistral 7B with the standard HIRO prompt. The other two LLMs, which were released since this work and which we suspect have been fine-tuned on citation tasks, successfully cite which input cluster they have used to generate parts of the output.}
    % \vspace*{-.2cm}
    \label{tab:hiro:citations}
\end{table*}

\todo{this table is too big, and needs mentioning in the main text}

\section{Limitations}

Since our approach identifies common opinions based on frequency of sentence encodings, we require a relatively large number of input sentences. We were not able to experiment with other popular datasets like Amazon \citep{10.1145/2872427.2883037}, Yelp \citep{meansum} or Rotten Tomatoes \citep{wang-ling-2016-neural} since these datasets only include a small number (usually 8) of input reviews.

HIRO can be trained without needing reference summaries, but the encoding space has a fixed capacity and is unlikely to generalize well to unseen domains. We welcome future work on extending the encoder or learning a domain-agnostic encoding space.

Although our experiments were limited to English, HIRO does not make any strong assumptions about the language of the reviews that it summarizes. However, it does make use of entailment models and tf-idf to select positive pairs for training, as well as LLMs for summary generation. Its application to other languages is therefore restricted to languages for which these resources are available. 


\section{Summary}

In this chapter, we propose HIRO, a modular method for unsupervised opinion summarization that uses a hierarchical index over sentences to select clusters of prevalent opinions. Our approach leverages pretrained Large Language Models to generate coherent and fluent summaries that are attributable and accurately reflect the popularity of opinions in the input reviews. Extensive experiments show that, as well as generating higher quality summaries, HIRO learns a more semantically distributed representation than competitive baselines.

While we limit our experiments to opinion summarization, we believe that HIRO demonstrates the efficacy of combining LLMs with more specialised models based on structured representations, and the approach could be usefully applied to a wide range of other retrieval-augmented generation tasks.

This chapter acts as the final piece of evidence in support of our core hypothesis; the discrete hierarchical encoding space directly enables attributable and scalable opinion summarisation. Building on \Cref{ch:hercules}, we show that the use of structured representations is compatible with LLMs. Using each approach on the subtasks for which they are best suited --- compressed structured representations for scalable content selection, LLMs for fluent language modelling --- allows us to achieve higher performance than a single model for the full task.

% \pagebreak

% \section{*Acknowledgements}

% We thank the action editor and anonymous reviewers for their constructive feedback. The authors also thank [...].




